PrIU: A Provenance-Based Approach for Incrementally Updating Regression Models

The ubiquitous use of machine learning algorithms brings new challenges to traditional database problems such as incremental view update. Much effort is being put in better understanding and debugging machine learning models, as well as in identifying and repairing errors in training datasets. Our focus is on how to assist these activities when they have to retrain the machine learning model after removing problematic training samples in cleaning or selecting different subsets of training data for interpretability. This paper presents an efficient provenance-based approach, PrIU, and its optimized version, PrIU-opt, for incrementally updating model parameters without sacrificing prediction accuracy. We prove the correctness and convergence of the incrementally updated model parameters, and validate it experimentally. Experimental results show that up to two orders of magnitude speed-ups can be achieved by PrIU-opt compared to simply retraining the model from scratch, yet obtaining highly similar models.

==> Sections/Introduction.tex <==
\section{Introduction}

%thing about real examples

%\struct{A few remarks about the data cleaning problem, dirty data, correct data.}
\eat{Data cleaning has been extensively studied in database communities in the last two decades \cite{dasu2003exploratory, rahm2000data,  chu2016data}, 
\val{I added a citation to FanGeerts Data Quality but it does not compile?!?}
whose accuracy can significantly influence the data analysis results and the following decision process. Currently data cleaning has gradually become an interactive and iterative process for data analysts \cite{krishnan2016towards} who need to alternate between analysis process and cleaning process and cooperate with other parties (e.g. IT staffs and data curators). Typical data cleaning problems includes how to determine which dirty data to be cleaned, how to evaluate the quality of the cleaning operations, how to reduce the latency of data cleaning process and how to repair the errors or noise data from the datasets, etc.. }
Data cleaning is essential for data analytics, and has been extensively studied by the database community~\cite{dasu2003exploratory, rahm2000data, fan2012quality, chu2016data}. 
The process is typically {iterative} and {interactive}, allowing data analysts to alternate between analysis and cleaning tasks, as well as to interact with other parties such as IT staff and data curators~\cite{krishnan2016towards}. Typical problems in data cleaning include determining which data is dirty, understanding how to repair errors, evaluating the quality of the cleaning operations, and speeding up
%the latency
the data cleaning process.


%\struct{What is special about cleaning training data?}
Many of these efforts have focused on SQL-based analytic workflows, and cannot handle the complexities introduced by machine learning algorithms, e.g. iterative computation and non-linear operations.
However, machine learning and other statistical analyses are  highly sensitive to dirty data, even when robust machine learning algorithms are used~\cite{chu2016data}. Dirty data in training datasets is especially problematic since it can result in erroneous models and thus totally counter-intuitive predictions for test datasets. \eat{Such problems become even worse in the face of other concerns, such as privacy and security~\cite{chu2016data}. \scream{Sue: I'm not sure what this last sentence means.}}

%how our work differs from existing data cleaning work
\eat{Both existing machine learning literature and database literature provide a series of solutions on how to detect and repair dirty data in training and test dataset \cite{krishnan2017boostclean, heidari2019holodetect} under the existence of different kinds of dirty data. For example, However, our work is orthogonal to existing error detection and repair works since we do not aim at providing a new solution for identifying dirty data. In this paper, we assume that the dirty data in the training dataset can be found by existing error detection solutions and our work targets at providing a new solution to speed up the following step, i.e. incrementally updating the machine learning model after the detected dirty are removed. So our contribution is to the data management associated with data cleaning, which ends up with a complementary tool in existing data cleaning pipeline to significantly reduce the latency and thus achieve the interactivity in the data cleaning process. Our focus is especially on propagating the effect of deleting training data to the corresponding updates of the model parameters. This is related to our previous approach to provenance. }
A number of techniques have therefore recently been proposed for detecting and repairing dirty data in training and test datasets, e.g., 
\cite{krishnan2017boostclean, heidari2019holodetect}. 
The work presented in this paper can be incorporated into data cleaning pipelines by assuming that dirty data in the training set has already been detected, and addresses the next step by providing a solution for incrementally updating the machine learning model after the dirty data has been removed.\footnote{The work presented here is not applicable to incremental insertions of new training samples, but it may be useful for \emph{modifications}, i.e., changing the values of some of the features (see the discussion
on future work  in Section~\ref{sec: conclusion}).} 
%Our contribution is therefore a complementary \val{better way to say that?} tool within the data cleaning pipeline, which can be used to reduce latency and thus enable interactivity in the data cleaning process. 
Our focus is on propagating the effect of deleting subsets of training data to the corresponding updates to the model parameters, and doing so efficiently.


Also, there has been an increasing need for privacy protection from recent laws, such as the General Data Protection Regulation (GDPR) \cite{GDPR}, which require companies and institutions that process personal data to delete user data upon users' request. If the deleted data are involved in the machine learning training process, their effect should be also removed from the trained ML models and thus the ML model parameters should be ``decrementally'' updated \cite{schelteramnesia}.  

%connection to interpretability of machine learning model
%\struct{This is related to what is called "influence" of one or more items in the training data on the model parameters.}
Another contribution of our approach is a better, more fine-grained, understanding of how the parameters of the learned model depend on the training data. For example, suppose the training data comes from several different sources and we wish
to understand how one of these sources affects the model.
% which has become increasingly challenging with the use of complex machine learning models, e.g. deep neural networks.
This is related to the notion of {\em interpretability}~\cite{doshi2017roadmap, poursabzi2018manipulating}.  One approach to interpretability that has been proposed in the machine learning community~\cite{koh2017understanding} is to develop an {\em influence function} to approximately quantify the influence of a single training sample on the model parameters and prediction results; this can also be used to estimate the model parameter change after the removal of a training sample. 
However, our results show (see Section~\ref{sec: experiment}) that extending the influence function approach
to multiple training samples (for example, all those coming from a given source) leads to very inaccurate models.
Searching for another approach, we note that interpretability can be seen as a \emph{provenance} question.
\eat{However, we demonstrate experimentally (see Section \ref{sec: experiment}) that this approach
leads to very inaccurate models when extended
%their method naively 
to handle the deletion of multiple training samples.}
\eat{not sure if we should say here 10\%}
%\val{I thought there is a naive way to extend their definition to multiple samples
%but this sacrifices accuracy?}\yinjun{yes, modified}
\eat{
As our experiments will demonstrate  using influence functions to estimate the change of model parameters is very inaccurate 
\val{this needs to be better explained}\yinjun{done by explaining that their approach is based on Talyor expansion}
when multiple training samples (say 10\% of training samples) are removed.}
% compared to expected updated model parameters, which is even harmful for the following prediction step.

% brief intro to data provenance and its connections to data cleaning and interpretability problem
%\struct{Incremental updates to model parameters. Relation with provenance.} 
%\val{Deletion propagation OK but how about insertions?}
\eat{
To achieve the goal of efficiently incrementally updating the model after the removal of {\em subsets} of training samples, we use {\em data provenance}~\cite{green2007provenance, green2010provenance, buneman2001and}. 
%which has been extensively studied in the last few decades 
%OK SUE I AM MOVING ELSEHWRE YOU HAVE THE INTRODUCTION
Data provenance can be used to track the dependency between input data and output data, upon which the reasoning can be conducted at finer-grain level. Such fine-grained analysis nature of data provenance has enabled incremental update support \cite{green2010provenance, ives2008orchestra} as well as interpretability support \cite{amsterdamer2011provenance} in database domain, both of which rely on provenance semiring model \cite{green2007provenance}. Provenance semiring model aims at propagating the provenance tokens associated with the input tuples through relational algebra operations such as join and union to the query result, which are extended to linear algebra operations such as matrix additions and multiplications in \cite{yan2016fine}. As \cite{buneman2019data} envisioned, it will be a promising area to utilize data provenance to provide interpretability for machine learning models.
}
====THE TEXT FROM HERE====

To achieve the goal of  incrementally updating the model after the removal of subsets of training samples, we therefore use {\em data provenance}~\cite{green2007provenance, green2010provenance, buneman2001and}.
Data provenance tracks the dependencies between input and output data; in particular, the provenance semiring model \cite{green2007provenance} can be used to enable incremental updates~\cite{green2010provenance, ives2008orchestra} as well as interpretability~\cite{amsterdamer2011provenance} in database queries.

\textbf{
[[[[as well as
interpretability~\cite{amsterdamer2011provenance} 
****??? This is the aggregates paper. I don't understand
why it is especially supporting interpretability?]]]}

This is done by propagating provenance tokens associated with the input tuples through relational algebra operations such as join and union to the query result.  
More recently, this has been extended to include linear algebra operations such as matrix addition and multiplication~\cite{yan2016fine}. 
As envisioned in~\cite{buneman2019data}, this is a first step in using data provenance to provide interpretability for machine learning models.


% highlight the difficulty to provide full-fledged solutions to general machine learning problem. 
\eat{Unfortunately, the existing provenance semiring model lacks the power of incremental updates over typical machine learning models due to the existence of non-linear operations in prevalent machine learning models, e.g. logistic regression model. To overcome this, we assume that gradient descent method (\gd) and its variants, i.e. stochastic gradient descent (\sgd) and mini-batch stochastic gradient descent (\minisgd) are used to derive the update rules in the training phase and we proposed the use of piecewise linear interpolation to convert the non-linear operations in the update rules into linear operations to facilitate the use of provenance in the following step.}
Unfortunately, the current provenance semiring model cannot be used for incremental updates over popular machine learning models such as logistic regression due to the use of non-linear operations. To overcome this, we assume that gradient descent (\gd) and its variants, i.e. stochastic gradient descent (\sgd) and mini-batch stochastic gradient descent (\minisgd), are used to compute the model parameters in the training phase iteratively. In this case, piecewise linear interpolation can be used to convert non-linear operations in the update rules into linear operations approximately, thereby facilitating the use of provenance.

\eat{
Considering the overhead of capturing and reasoning over provenance and the model complexity in general machine learning pipelines, it is difficult to achieve efficient incremental updates over general machine learning model by applying the update rule-based provenance support strategies mentioned above. Even for some simple machine learning models such as logistic regression, designing full-fledged solutions is also a non-trivial task. So in this paper, we will present an efficient incremental model update strategy i.e. \pro\ and its optimized version \proopt\ for simple machine learning models i.e. linear regression model and (binary and multinomial) logistic regression model and leave the exploration for more complicated models for future work. 
}

In linear and logistic regression, gradient descent is used to iteratively calculate the model parameters.
In each iteration, a formula called the ``update rule" uses the gradient of the objective function to update the model parameters.  This is done by taking the sum of the derivatives over {\em all} the training samples. After removing $k$ training samples, the naive solution for updating the model parameters would be to sum up the derivatives of the {\em remaining} training samples  -- which is still large since $k$ is typically far smaller than the total number of training samples. To speed up the computation, for linear regression we are able to cache {\em intermediate results} in the gradient expression over all the training samples which are {\em free of model parameters} (The intermediate results in the update rule of linear regression are $\textbf{X}^T\textbf{X}$ and $\textbf{X}^T\textbf{Y}$. 
); thus the intermediate results
%before the removal requests, 
only include information from the training samples. 
We can then simply subtract the {\em removed samples} from the intermediate results in the update rule. We do this by tracking the provenance of intermediate results, and ``zeroing out'' the removed samples in the provenance expression for each intermediate result.  This reflects the idea of deletion propagation in {\em provenance}~\cite{green2007provenance}.
% and can be easily realized in linear regression where the 
However for logistic regression,  it is not straightforward to find model-free intermediate results to cache during the update rule due to the existence of non-linear operations.
To overcome this, we use {\em piecewise linear interpolation} to linearize these operations so that the expression with model parameters and the expression with training data become ``independent'' of each other; thus the latter expression becomes the intermediate result that we want. We can also prove that the errors produced by the linearization approximation are small. 

===TO HERE IS TO BE REPLACED WITH BELOW==

==BEGINNING OF PROPOSED REPLACEMENT===

To achieve the goal of incrementally updating the model after the
removal of subsets of training samples, we use {\em data
provenance}~\cite{green2007provenance,buneman2001and,CheneyCT09}.  
In general, data provenance tracks the dependencies between
input and output data; in particular, the \emph{provenance semiring framework}
\cite{green2007provenance,GreenT17}
has been used for applying
incremental updates (specifically deletions)
to views, and more generally, through schema 
mappings~\cite{ives2008orchestra}.

In the semiring framework, output data is annotated with \emph{provenance
polynomials} expressed in terms of provenance tokens that annotate
input data thus making deletion propagation straightforwardly efficient.
%This is done by propagating provenance tokens associated with the
%input tuples through relational algebra operations such as join and
%union to the query result.[[[NO NEED HERE; THIS IS EXPLAINED IN MORE 
%DETAIL IN SECTION 4.1]]]  
The framework has proven quite versatile, allowing for extensions 
to powerful query languages (see references in~\cite{GreenT17}).
Most relevant to the present paper, the framework has been extended to
include the basic linear algebra operations: matrix addition and
multiplication~\cite{yan2016fine} (which was mentioned 
in~\cite{buneman2019data} as a first step in using data
provenance for interpretability of machine learning models).
In this extension, as in ~\cite{amsterdamer2011provenance}, the
provenance polynomials play the role of scalars and multiplication
with scalars plays the role of annotating matrices and vectors with
provenance.


In this paper we use the extension of the semiring framework to
basic linear algebra in order to track the provenance of input
samples through the training of logistic regression and linear
regression models using iterative gradient-based methods (GBMs).
In each iteration, we have a gradient-based ``rule'' that updates the 
model parameters. We can annotate the gradient update rule with 
provenance polynomials 
when it is expressed using matrix addition and multiplication. This is
the case when using GBM in linear regression. For logistic regression
we achieve this via piecewise linear interpolation of the non-linear
components in the gradient update rule.

In addition to allowing provenance tracking, the linearization of the
gradient update rule also allows us to separate the contributions of
the training samples from the contributions of the model parameters
(from the previous iteration).  As a result, the effect of deleting
training samples upon the gradient update rule can be obtained by
setting the provenance tokens corresponding to those samples to zero.
To speed up computation, we are able, for both linear and logistic
regression, to cache, between iterations, intermediate results that
capture only the contribution of the training samples, annotated with
provenance. Propagating the deletions of some of the samples then
comes down to subtracting a portion of these intermediate results.  An
additional subtlety for logistic regression is that the piecewise
linear interpolation uses coefficients which are different in
different iterations and hence need to be tracked in the computation.


==END OF PROPOSED REPLACEMENT==

We illustrate below how provenance can be used to incrementally update the model parameters after removing a subset of training data.

\begin{example}
%\subsection{Example}
Consider the UCI Skin Segmentation  \footnote{\url{https://www.csie.ntu.edu.tw/~cjlin/libsvmtools/datasets/binary.html#skin_nonskin}} dataset, which is used to classify pixels in images of faces as skin or not-skin using RGB values along with other features such as gender and race. A training dataset containing three samples 
%(which is unrealistically small) 
is shown in Figure \ref{fig: example} (ignore the last column for the moment). For simplicity, we only show the feature values for R, G, B attributes as well as the label (skin\_or\_not) for each sample. 

\begin{figure}[!htb]
\includegraphics[width=0.45\textwidth, height=0.25\textwidth]{Figures/example.png}
\caption{UCI Skin Segmentation training dataset example}\label{fig: example}
\end{figure}

Suppose that logistic regression with stochastic gradient descent (SGD) is used during the training phase, resulting in the vector of model parameters $(0.423, 0.6, -0.9,...)$ shown in the middle of the figure.
%Figure \ref{fig: example}.  
When running the model over the test dataset, it turns out that the accuracy is low, only 60\%. After consulting with experts who are familiar with the dataset, the first sample is discovered to be an error and is removed from the training phase. Rather than rerunning the logistic regression over the modified training dataset, we update the model parameters directly using provenance.

We start by annotating each training sample with a unique provenance token, e.g. $p_1, p_2, p_3$ for the three samples.
%in Figure \ref{fig: example}.
The value of $p_i(i=1,2,3)$ can be 1 or 0 representing the existence or non-existence of the corresponding training sample.  During the training phase over the original (dirty) dataset, the provenance tokens are propagated through the SGD computation. As a result, the model parameters (i.e. $(0.423, 0.6, -0.9,...)$) will be broken into different pieces, each of which is associated with some {\em joint} combination of the provenance tokens (the {\em tensor product} as will be seen later). For example, in Figure \ref{fig: example}, one such tensor product is $(0.134, 0.472, -0.28,\dots)*p_1$, which intuitively means that if only the first sample exists, the model parameters will be $(0.134, 0.472, -0.28,\dots)$. We can then ``remove'' the first sample by setting $p_1$ to 0 and $p_2$, $p_3$ to 1, and thus derive the updated model parameters, $(0.84, -0.06, 0.32,\dots)$ (shown at the bottom of the figure). Note that the model does not need to be retrained over the reduced training dataset; the model parameters are updated directly.  This new model now has a much higher test accuracy (90\%), similar to that achieved by retraining from scratch.
\end{example}



One challenge of using provenance to enable incremental updates over machine learning models is the overhead, due not only to capturing and reasoning over provenance but to the model complexity in machine learning pipelines.
As a result, it is difficult to achieve {\em efficient} incremental updates by straighforwardly applying the update rule-based provenance strategies illustrated above. 
%Even for some simple machine learning models, such as logistic regression, designing full-fledged solutions is non-trivial. 
We therefore develop an {\em efficient incremental model update strategy}, \pro, and its optimized version, \proopt, for several simple machine learning models. The models include linear regression and (binary and multinomial) logistic regression.

Extending this to more complicated models is left for future work. A possible wider target, especially for the 
optimization ideas embodied in \proopt\ is the class of \emph{generalized additive models} (GAM)~\cite{hastie1986gam}.
Note also that 1) the multinomial logistic regression model represents the last layer, i.e. the softmax layer, 
of a typical deep neural network models; and 2) one of the most widely used activation functions in 
\emph{deep neural network models (DNNs)} is the sigmoid function, which is the same as the non-linear operation in the logistic regression model\eat{; and 3) another typical activation function in DNNs is the ReLU function, which is a segmented linear function and thus closely related to piecewise linear interpolation used in our approach}.
This suggests DNNs as another future target.

\textbf{Contributions} of this paper include:
%\vspace*{-1mm}
\begin{enumerate}
    \item A theoretical framework which enables data provenance to be tracked and used for very fast incremental model updates when subsets of training samples are removed.  The framework extends the approach in~\cite{green2007provenance, green2010provenance,yan2016fine} to  linear regression and (binary and multinomial) logistic regression models.
    
    \item Analytical results showing the convergence and accuracy of the updated model parameters which are approximately computed by applying piecewise linear interpolation over the non-linear operations (in logistic regression) in the model parameter update rules. 
    
    \item Efficient provenance-based algorithms, \pro\ and \proopt, which achieve very fast model updates after removing subsets of training samples through efficient matrix operations, using the singular value cdecomposition to reduce the dimenension of the intermediate results, using an incremental eigenvalue update approach to avoid expensive repetitive computation, and terminating provenance tracking early when provenance expressions stabilize. 
     
    \item Extensive experiments showing the effectiveness and accuracy of \pro\ and \proopt\ in incrementally updating the linear regression and logistic regression models compared to the straightforward approach of retraining from  scratch and compared to implementing an extension of the influence function in \cite{koh2017understanding}.
    
    \item Extending current work on interpretability by enabling the understanding the effect of removing {\em subsets} of the training data, rather than just a single training sample.
    
\eat{
- model of provenance for linear matrix operations -- WHAT ARE THESE
- use of this model to linear regression as well as a linearized version of logistic regression based on approximation
- correctness analysis: proof of convergence of resulting provenance expression whenever the model parameter w converges, proof on bound between the real and approximated model parameters
- application to cleaning, understanding influence of inputs on model
- speed up computation (optimization) of model update under deletion
}


\end{enumerate}


The remainder of the paper is organized as follows. In Section \ref{sec: related_work}, we describe  related work in incremental model maintenance, data provenance, data cleaning, and machine learning model interpretability. Section \ref{sec: prl} reviews the basic concepts of linear regression, logistic regression, and piecewise linear interpolation. The theoretical development of how to use provenance in the update rules of linear regression and logistic regression is presented in Section \ref{sec: model}, and its implementation provided in Section \ref{sec: implementation}. Experimental results showing the feasibility of our approach compared to other solutions are presented in Section \ref{sec: experiment}. We conclude in Section \ref{sec: conclusion}.


To our knowledge, this is the first work to use provenance 
%(in particular, the provenance semiring model) 
for the purpose of incrementally updating machine learning model parameters.  
\eat{
through gradient-based method in the context of cleaning dirty data and interpretability of machine learning models.}


\eat{Extending this to more complicated models is left for future work. But considering the similarity between multinomial logistic regression and some portions of more complicated models, e.g. multinomial logistic regression is the same as the softmax layer of deep neural network models, we believe that the solutions proposed in this paper can be potential used in those models.}
%\susan{This is now repetitive of the above.}\yinjun{removed}


\medskip







\eat{
\susan{This remains to be completed... contributions and outline of paper?}
\eat{If lot of parameters, the performance of our approach is bad.  Sort of related to the number of features.  Deep learning has a lot of parameters.}
%approaches: SGD/GD, approximation, 
highlight the novelty of our contributions. This is the first work to marry provenance and machine learning training phase for the purpose of efficient incremental updates

\struct{
\begin{itemize}
    \item Related work
    \item Preliminaries which learning model (linear, logistic, multinomial logistic); 
    which iterative algorithm for parameter learning (SGD, miniSGD,...)
    \item Model: provenance decoration of iterative algo; separate issue: linearize logistic regression.
    \item "Implementation": further detail the algorithm
    \item Experimental evaluation.
\end{itemize}
}




}

==> Sections/alt-4-1.tex <==
\subsection{Provenance annotations and semantics}
\label{ssec: provenance_annotation}

In the semiring 
framework~\cite{green2007provenance,amsterdamer2011provenance,GreenT17}
one begins by annotating input data with elements of a set $X$ of 
\emph{provenance tokens}. These annotations are then propagated through 
query operators as they combine according to 
two operations: ``$+$'' that records \emph{alternative} use of information, 
as in relational union or projection, and  ``$\cdot$'', that records 
\emph{joint} use of information, as in relational join. With these, the 
annotations become  \emph{provenance polynomials} whose indeterminates are 
the tokens in $X$ and whose coefficients are natural numbers. We denote the 
set of polynomials by $\mathbb{N}[X]$.

In the extension of the framework to matrix algebra~\cite{yan2016fine},
annotation formally becomes a 
\emph{multiplication of vectors with scalars} as in linear
algebra. The role of scalars is played by provenance polynomials and 
the role of vectors, of course, is played by matrices (generalizing their
row vectors and the transposes of these).

\reminder{Not sure if we want to include this: This further generalizes the
use of annotation as scalar multiplication in the work on provenance for 
aggregation~\cite{amsterdamer2011provenance}.}

\emph{Matrices annotated with provenance polynomials} form a nice
algebraic structure that extends matrix multiplication and
addition. We denote multiplication with scalars by ``$*$'' writing
$\mathfrak{p}*\mathbf{A}$ for the matrix $\mathbf{A}$ annotated with the
provenance polynomial $\mathfrak{p}$. For space reasons we cannot repeat
here the technical development in~\cite{yan2016fine}, however, we mention
an crucial algebraic property of annotated matrix multiplication, which
also illustrates combining provenance in joint use:
$$
(\mathfrak{p}_1 * \mathbf{A}_1)(\mathfrak{p}_2 * \mathbf{A}_2) = 
(\mathfrak{p}_1 \cdot \mathfrak{p}_2)*(\mathbf{A}_1\mathbf{A}_2)
$$


\eat{
which is based on a generalization of the standard construction of
{\em tensor product}.

Let $(\mathcal{M}, +, \cdot, 0, I)$ be the {\em many-sorted} ring of matrices of various dimensions
and let $(K, +_K, \cdot_K, 0_K, 1_K)$ be a commutative semiring (we only use the semiring of provenance polynomials~\cite{green2007provenance}). We denote by $K \bigotimes \mathcal{M}$ the generalized
tensor product of $K$ and $\mathcal{M}$~\cite{yan2016fine}. 
The construction yields a (non-commutative) ring $(K \bigotimes \mathcal{M},+\cdot,0,I)$ together with a multiplication with scalars from $K$
that we denote by $*$  such that $\forall k, k_1, k_2 \in K, A_1, A_2, A_3 \in K \bigotimes \mathcal{M}$, the following equalities hold:
\begin{enumerate}
    \item $k * (A_1 + A_2) = k* A_1 + k * A_2$
    \item $k * 0 = 0$
    \item $(k_1 +_K k_2) * A = k_1* A + k_2* A$
    \item $0_K * A = 0$
    \item $(k_1 \cdot_K k_2) * A = k_1 * (k_2 * A)$
    \item $1_K * A = A$
    \item $(k_1 * A_1)(k_2 * A_2) = (k_1 \cdot k_2)*(A_1A_2)$
\end{enumerate}
The basic elements of $K \bigotimes \mathcal{M}$ have (modulo the standard equivalences used 
in the tensor product construction) the form $k * M$ where $k\in K$ is,
for example, a provenance polynomial, and $M$ is a matrix (including $m\times1$, $1\times n$ and even $1\times 1$ matrices). Note that the ring of matrices $\mathcal{M}$ is \emph{embedded} into
$K \bigotimes \mathcal{M}$ as every matrix $M$ can be seen as $1_K * M \in K \bigotimes \mathcal{M}$.
%provenance tokens for each row of the input, leading to the provenance tokens for the entire matrix or vector
}

We apply this framework to tracking input training samples through
$\gbm$'s in which the update involves only matrix multiplication and
addition. Let the training dataset be $(\mathbf{X},\mathbf{Y})$ where 
$\mathbf{X}$ is an $n\times m$ feature matrix and $\mathbf{Y}$ is
an $n\times 1$ column vector of sample labels.  For $i=1,\ldots, n$
we annotate every sample
$(\textbf{x}_i,y_i)$ ($\textbf{x}_i$ and $[y_i]$ are the $i$'th rows
in $\mathbf{X}$ respectively $\mathbf{Y}$) with a distinct provenance 
token $p_i$. Next, we decompose $\mathbf{X}$ and $\mathbf{Y}$ as algebraic
expressions in terms of $p_1*\textbf{x}_1, \ldots, p_n*\textbf{x}_n, 
p_1*[y_1], \ldots, p_n*[y_n]$ and some matrices made up of the reals 0 and 1.
These ``helper'' matrices are annotated with the provenance polynomial 
$1_{\mathbf{N}[X]}$ 
(has a term of degree zero which is the natural number 1) meaning
``always available, no need to track''.
We illustrate with the provenance-annotated $\mathbf{X}$ when $n=2$:
$$
\mathbf{X} ~=~ (1_{\mathbf{N}[X]} * \begin{bmatrix}
                                 1\\
                                 0
                                 \end{bmatrix})
           (p_1*\mathbf{x}_1) ~+~ 
               (1_{\mathbf{N}[X]} * \begin{bmatrix}
                                 0\\
                                 1\\
                                 \end{bmatrix} 
          (p_2*\mathbf{x}_2) ~=~
$$
$$
~=~ (p_1 *\begin{bmatrix}
         \mathbf{x}_1\\
         0\ldots0
         \end{bmatrix}) ~+~
    (p_2 *\begin{bmatrix}
         0\ldots0\\                
            \mathbf{x}_2
         \end{bmatrix}) 
$$

When $\mathbf{X}$ is transposed, a similar decomposition applies
in terms of the annotated column vectors $p_i*\textbf{x}_i^T$.
\reminder{Skipping this: The more general annotation technique 
of~\cite{yan2016fine} can annotate columns as well} 
We also note that the algebra of annotated matrices follows the
same laws as the usual matrix algebra. Consequently, we can perform
in the algebra of provenance-annotated matrices the calculations involved 
in the gradient-based update rules. For illustration, a calculation involving
$\mathbf{X}$ that without
provenance takes the form $\sum_{i=1}^n a_i\mathbf{x}_i\mathbf{x}_i^T$ 
where $a_i$ are some real numbers becomes with provenance annotations
$$
\sum_{i=1}^n (1_{\mathbf{N}[X]}*[a_i])(p_i*\mathbf{x}_i)(p_i*\mathbf{x}_i^T)
~=~ 
\sum_{i=1}^n p_i^2*(a_i\mathbf{x}_i\mathbf{x}_i^T)
$$

%for the input training dataset ($\textbf{X}, \textbf{Y}$), we only annotate every row (i.e. every sample) of $\textbf{X}$ and $\textbf{Y}$ with provenance tokens without annotating the columns, which is
%is a simplified version of the provenance model of \cite{yan2016fine} 
%but is enough for the purpose of incremental updates to the training of machine learning models. We also assume that for every sample ($\textbf{x}_i, \textbf{y}_i$), the provenance tokens $p_i$
%are same for both $\textbf{x}_i$ and $\textbf{y}_i$, which results in the following provenance annotated training dataset:

\eat{
\begin{align}\label{eq: training_data_x_with_provenance}
    \begin{split}
    \textbf{X} &= \begin{bmatrix}
p_1 * \textbf{x}_1, p_2 * \textbf{x}_2, \dots, p_n * \textbf{x}_n
\end{bmatrix}^T\\
\textbf{Y} &= \begin{bmatrix}
p_1 * y_1, p_2 * y_2, \dots, p_n * y_n \end{bmatrix}^T 
    \end{split}
\end{align}
% \begin{equation}\label{eq: training_data_x_with_provenance}
% \textbf{X} = \begin{bmatrix}
% p_1 * \textbf{x}_1^T\\
% p_2 * \textbf{x}_2^T\\
%  \dots\\
% p_n * \textbf{x}_n^T
% \end{bmatrix}
% \textbf{Y} = \begin{bmatrix}
% p_1 * y_1\\
% p_2 * y_2\\
%  \dots\\
% p_n * y_n
% \end{bmatrix}
% \end{equation}

%tensor product, semi-module
% Based on the ideas from \cite{yan2016fine}, we can further define provenance token propagation rules through the vector operations since all the iterative update rules in Equation \ref{eq: mini_sgd_instantiation_approx} only involve vector addition and multiplication
}. 

\eat{
Based on the annotations for $\textbf{X}$ and $\textbf{Y}$, the provenance expression for typical matrix operations can be derived, which is exemplified as below:
\scream{Yinjun: proposed one example on how to use semiring model below}
\begin{example}
The provenance expression of $\sum_{i=1}^n a_i\textbf{x}_i\textbf{x}_i^T$ and $\sum_{i=1}^n b_i\textbf{x}_i y_i$ is:
\begin{align}\label{eq: example_provenance}
    \begin{split}
        \mathscr{P}(\sum_{i=1}^n a_i\textbf{x}_i\textbf{x}_i^T) &= \sum_{i=1}^n p_i^2*(a_i\textbf{x}_i\textbf{x}_i^T)
    \end{split}
\end{align}
\begin{align}\label{eq: example_provenance2}
    \begin{split}
        \mathscr{P}(\sum_{i=1}^n b_i\textbf{x}_iy_i) &= \sum_{i=1}^n p_i^2*(b_i\textbf{x}_i y_i)
    \end{split}
\end{align}

where $\mathscr{P}(*)$ represents the provenance expression of some matrix expression. Since each $a_i\textbf{x}_i\textbf{x}_i^T$ is the multiplications between $a_i$, $\textbf{x}_i$ and $\textbf{x}_i^T$, which can be expressed as tensor products $1_k*a_i$ ($a_i$ is a constant), $p_i*\textbf{x}_i$ and $p_i*\textbf{x}_i^T$ as the consequence of provenance annotations, then Equation \ref{eq: example_provenance} can be regarded as the result of applying the rule (\ref{eq: associativity}), i.e.  $(1_k*a_i)(p_i*\textbf{x}_i)(p_i*\textbf{x}_i^T) = (1_k\cdot_K p_i \cdot_K p_i) (a_i \textbf{x}_i\textbf{x}_i^T) = p_i^2*(a_i \textbf{x}_i\textbf{x}_i^T)$. Equation \ref{eq: example_provenance2} can be derived in a similar way.
\end{example}
}

\eat{
Since matrices can be embedded in $K \bigotimes \mathcal{M}$, the update rules under \gbm\ 
correspond to update rules in $K \bigotimes \mathcal{M}$ involving matrices "with provenance".
}

And here is the provenance-annotated expression for the update rule 
of linear regression (i.e. Equation~\ref{eq: mini_sgd_linear_regression}):
\begin{align}\label{eq: mini_sgd_linear_regression_provenance}
    \begin{split}
        &\mathcal{W}^{(t+1)} \leftarrow [(1-\eta_t\lambda)(1_k * \eat{\cdot} \textbf{I}) \\ &-\frac{2\eta_t}{\mathcal{P}^{(t)}} \sum_{i \in \mathscr{B}^{(t)}} p_i^2 * \eat{\cdot}
        \textbf{x}_i\textbf{x}_i^T] \mathcal{W}^{(t)} + \frac{2\eta_t}{\mathcal{P}^{(t)}} \sum_{i\in \mathscr{B}^{(t)}}p_i^2 * \eat{\cdot} 
        \textbf{x}_iy_i
    \end{split}
\end{align}
% Ideally, with the iteration proceeds, the provenance for the model parameter can be also computed iteratively. To conduct incremental updates by removing the samples of interest (say $\textbf{x}_i$), we can simply setting $p_i$ as 0 and get the updated 
%apply idempodence over *_K, map the simplified version of provenance expression to the incremental updated model parameters.
\noindent
where $\mathcal{W}^{(t)}$ represents the provenance-annotated expression for model parameter $\textbf{w}^{(t)}$ while $\mathcal{P}^{(t)}$ represents the provenance-annotated expression
for the batch number $B$ at the $t^{\mathrm{th}}$ iteration, i.e. $\mathcal{P}^{(t)} = \sum_{i \in \mathscr{B}^{(t)}} p_i * \eat{\cdot} 1$.
%\val{Three kinds of B may be too much. Consider using $\mathcal{P}^{(t)}$ instead of $\mathcal{B}^{(t)}$.}
%\yinjun{done}

%\val{we need to explain what is division by a provenance expression 
%since $\mathcal{B}$ appears in a denominator}. 
In the provenance semiring framework there is no division operation for provenance expressions,
although a division-like symbol has been used in Equation~\ref{eq: mini_sgd_linear_regression_provenance}
for notational purposes. In fact, in the context of the incremental update problem, once the subset of training samples (say ($\Delta \textbf{X}, \Delta \textbf{Y}$)) to be removed is determined, the corresponding provenance tokens will be set as $0_{K}$ 
% (say all the provenance tokens except $\{p_{i_1}, p_{i_2}, \dots, p_{i_z}\}$ are zeros due to the updates), 
and thus the number of non-zero tensor products in $\mathcal{P}^{(t)}$ can be determined, which also represents the size of the remaining samples in each min-batch 
%after the removal operation 
(denoted by $\increB^{(t)}$). So we can replace $\mathcal{P}^{(t)}$ with $\increB^{(t)}$ in the update rule that
gives $\mathcal{W}^{(t+1)}$, i.e.:
\begin{align}\label{eq: mini_sgd_linear_regression_provenance_update}
    \begin{split}
        &\increprov^{(t+1)} \leftarrow [(1-\eta_t\lambda)(1_K * \eat{\cdot} \textbf{I}) \\
        &-\frac{2\eta_t}{\increB^{(t)}} \sum_{\substack{ i \in \mathscr{B}^{(t)} \\, \textbf{x}_i \not\in \Delta \textbf{X}}} p_i^2 * \eat{\cdot} \textbf{x}_i\textbf{x}_i^T] \increprov^{(t)}+ \frac{2\eta_t}{\increB^{(t)}} \sum_{\substack{ i \in \mathscr{B}^{(t)} \\, \textbf{x}_i \not\in \Delta \textbf{X}\\, y_i \in \Delta \textbf{Y}}}p_i^2 * \eat{\cdot} \textbf{x}_iy_i
    \end{split}
\end{align}

\scream{Val: is there a typo with $y\in\Delta Y$?
But I don't think we should show this.}

Now suppose $\increprov^{(0)} = 1_K * \eat{\cdot} \textbf{w}^{(0)}$ \eat{represent number of non-zero provenance tokens in current batch}, then by induction we can observe that $\increprov^{(t)}$ should be the sum of multiple tensor products, each of which should be in the form of $P*\textbf{u}$ where $\textbf{u}$ is a matrix associated with a provenance monomial $P$ ($P= p_{j_1}^{r_1}p_{j_2}^{j_2}p_{j_3}^{r_3}\dots p_{j_k}^{r_k}$ and $r_i (i=1,2,\dots,k)$ is a natural number). Intuitively speaking, $P*\textbf{u}$ represents how the combinations of $r_1$ copies of ${j_1}^{\mathrm{th}}$ sample, $r_2$ copies of ${j_2}^{\mathrm{th}}$ sample, \dots and $r_k$ copies of ${j_k}^{\mathrm{th}}$ contribute to the model parameter where ${j_1}^{\mathrm{th}}, {j_2}^{\mathrm{th}}\dots, {j_k}^{\mathrm{th}}$ sample should not be in $\Delta \textbf{X}$.

Then by setting $p_i$ as 1, we can get the update rule to compute the updated model parameters as below:
\begin{align}\label{eq: mini_sgd_linear_regression_para_update}
    \begin{split}
        \increw^{(t+1)}& \leftarrow [(1-\eta_t\lambda)\textbf{I} -\frac{2\eta_t}{\increB^{(t)}} \sum_{\substack{ i \in \mathscr{B}^{(t)} \\, \textbf{x}_i \not\in \Delta \textbf{X}}} \eat{\cdot} \textbf{x}_i\textbf{x}_i^T] \increw^{(t)}\\
        &+ \frac{2\eta_t}{\increB^{(t)}} \sum_{\substack{ i \in \mathscr{B}^{(t)} \\, \textbf{x}_i \not\in \Delta \textbf{X}, y_i \in \Delta \textbf{Y}}}\eat{\cdot} \textbf{x}_iy_i
    \end{split}
\end{align}

which simply sum up the matrices from each tensor product on the right-hand side of Equation \ref{eq: mini_sgd_linear_regression_provenance_update}.

\eat{. are updated iteratively as the iteration proceeds. To conduct incremental deletion over the model parameters $\textbf{w}^{(t)}$ by removing the samples of interest (say $\textbf{x}_{i_1}, \textbf{x}_{i_2}, \dots, \textbf{x}_{i_z}$), we can simply setting $p_{i_1}, p_{i_2}, \dots, p_{i_z}$ as $0_K$ to eliminate the effect of those samples and setting other provenance tokens as $1_K$ at the same time.}
















\eat{
Unlike the more general annotation technique of~\cite{yan2016fine}, for the input training dataset ($\textbf{X}, \textbf{Y}$), we only annotate every row (i.e. every sample) of $\textbf{X}$ and $\textbf{Y}$ with provenance tokens without annotating the columns, which is
%is a simplified version of the provenance model of \cite{yan2016fine} but is 
enough for the purpose of incremental updates to the training of machine learning models. We also assume that for every sample ($\textbf{x}_i, \textbf{y}_i$), the provenance tokens $p_i$~\cite{green2007provenance,yan2016fine}
are same for both $\textbf{x}_i$ and $\textbf{y}_i$, which results in the following provenance annotated training dataset:

\begin{equation}\label{eq: training_data_x_with_provenance}
\textbf{X} = \begin{bmatrix}
p_1 * \textbf{x}_1^T\\
p_2 * \textbf{x}_2^T\\
 \dots\\
p_n * \textbf{x}_n^T
\end{bmatrix}
\textbf{Y} = \begin{bmatrix}
p_1 * y_1\\
p_2 * y_2\\
 \dots\\
p_n * y_n
\end{bmatrix}
\end{equation}

%tensor product, semi-module
% Based on the ideas from \cite{yan2016fine}, we can further define provenance token propagation rules through the vector operations since all the iterative update rules in Equation \ref{eq: mini_sgd_instantiation_approx} only involve vector addition and multiplication. 

Since matrices can be embedded in $K \bigotimes \mathcal{M}$, the update rules under \gbm\ 
correspond to update rules in $K \bigotimes \mathcal{M}$ involving matrices "with provenance". 
For example, after annotating 
each training sample in $(\textbf{X}, \textbf{Y})$ with provenance tokens as above for the update rule of linear regression, Equation~\ref{eq: mini_sgd_linear_regression} becomes:
\begin{align}\label{eq: mini_sgd_linear_regression_provenance}
    \begin{split}
        \mathcal{W}^{(t+1)}& \leftarrow ((1-\eta_t\lambda)(1_k * \eat{\cdot} \textbf{I}) -\frac{2\eta_t}{\mathcal{P}^{(t)}} \sum_{i \in \mathscr{B}^{(t)}} p_i^2 * \eat{\cdot}
        \textbf{x}_i\textbf{x}_i^T) \mathcal{W}^{(t)}\\
        &+ \frac{2\eta_t}{\mathcal{P}^{(t)}} \sum_{i\in \mathscr{B}^{(t)}}p_i^2 * \eat{\cdot} 
        \textbf{x}_iy_i\\
    \end{split}
\end{align}
% Ideally, with the iteration proceeds, the provenance for the model parameter can be also computed iteratively. To conduct incremental updates by removing the samples of interest (say $\textbf{x}_i$), we can simply setting $p_i$ as 0 and get the updated 
%apply idempodence over *_K, map the simplified version of provenance expression to the incremental updated model parameters.
\noindent
where $\mathcal{W}^{(t)}$ represents the provenance-annotated expression for model parameter $\textbf{w}^{(t)}$ while $\mathcal{P}^{(t)}$ represents the provenance-annotated expression
for the batch number $B$ at the $t^{\mathrm{th}}$ iteration, i.e. $\mathcal{P}^{(t)} = \sum_{i \in \mathscr{B}^{(t)}} p_i * \eat{\cdot} 1$.
%\val{Three kinds of B may be too much. Consider using $\mathcal{P}^{(t)}$ instead of $\mathcal{B}^{(t)}$.}
%\yinjun{done}

%\val{we need to explain what is division by a provenance expression 
%since $\mathcal{B}$ appears in a denominator}. 
In the provenance semiring framework there is no division operation for provenance expressions,
although a division-like symbol has been used in Equation~\ref{eq: mini_sgd_linear_regression_provenance}
for notational purposes. In fact, in the context of the incremental update problem, once the subset of training samples to be removed is determined, the corresponding provenance tokens will be set as $0_{K}$ (say all the provenance tokens except $\{p_{i_1}, p_{i_2}, \dots, p_{i_z}\}$ are zeros due to the updates), and thus the number of non-zero tensor products in $\mathcal{P}^{(t)}$ can be determined, which also represents the size of the remaining samples in each batch 
%after the removal operation 
(denoted by $\increB^{(t)}$). So we can replace $\mathcal{P}^{(t)}$ with $\increB^{(t)}$ in the update rule that
gives $\mathcal{W}^{(t+1)}$, i.e.:

\begin{align}\label{eq: mini_sgd_linear_regression_provenance_update}
    \begin{split}
        \increprov^{(t+1)}& \leftarrow ((1-\eta_t\lambda)(1_K * \eat{\cdot} \textbf{I}) \\
        &-\frac{2\eta_t}{\increB^{(t)}} \sum_{\substack{ i \in \mathscr{B}^{(t)} \\ i \in \{{i_1}, {i_2}, \dots, {i_z}\}}} p_i^2 * \eat{\cdot} \textbf{x}_i\textbf{x}_i^T) \increprov^{(t)}\\
        &+ \frac{2\eta_t}{\increB^{(t)}} \sum_{\substack{ i \in \mathscr{B}^{(t)} \\ i \in \{{i_1}, {i_2}, \dots, {i_z}\}}}p_i^2 * \eat{\cdot} \textbf{x}_iy_i
    \end{split}
\end{align}

Now suppose $\increprov^{(0)} = 1_K * \eat{\cdot} \textbf{w}^{(0)}$ \eat{represent number of non-zero provenance tokens in current batch}, then by induction we can observe that $\increprov^{(t)}$ should be the sum of multiple tensor products, each of which should be in the form of $P*\textbf{u}$ where $\textbf{u}$ is a matrix associated with a provenance monomial $P$ ($P= p_{j_1}^{r_1}p_{j_2}^{j_2}p_{j_3}^{r_3}\dots p_{j_k}^{r_k}$ and $p_{j_t} \in \{p_{i_1}, p_{i_2}, \dots, p_{i_z}\}$ and $r_i (i=1,2,\dots,k)$ is a natural number). Intuitively speaking, $P*\textbf{u}$ represents how the combinations of $r_1$ copies of ${j_1}^{\mathrm{th}}$ sample, $r_2$ copies of ${j_2}^{\mathrm{th}}$ sample, \dots and $r_k$ copies of ${j_k}^{\mathrm{th}}$ contribute to the model parameter.
}


\eat{. are updated iteratively as the iteration proceeds. To conduct incremental deletion over the model parameters $\textbf{w}^{(t)}$ by removing the samples of interest (say $\textbf{x}_{i_1}, \textbf{x}_{i_2}, \dots, \textbf{x}_{i_z}$), we can simply setting $p_{i_1}, p_{i_2}, \dots, p_{i_z}$ as $0_K$ to eliminate the effect of those samples and setting other provenance tokens as $1_K$ at the same time.}



==> Sections/alt-intro.tex <==

\section*{ALTERNATIVE TITLE:}

\textsc{PrIU: Assisting interpretability of regression 
models with provenance-based incremental updates}

\section*{NEW Introduction}

In databases terminology, this paper is about \emph{efficient incremental
view update}, specifically about using provenance annotations to
propagate deletions from the input data. However,
the views that we consider are \emph{regression models} (linear and
binomial/multinomial logistic regression) and the input data consists
of the samples used to train these models.

We target applications in which machine learning engineers must perform 
\emph{repeated retraining} of models using multiple different subsets 
of a training dataset. This occurs in the data-driven approach to 
discover \emph{factors of interpretability}~\cite{doshi2017roadmap}
and can be used, for example, to understand relationships between
samples with certain feature characteristics and model behavior.
This can also occur in 
\emph{model debugging}~\cite{krishnan2016activeclean,KangRBZ18,heidari2019holodetect} 
and in \emph{deletion diagnostics}~\cite{cook1977detection}
when a more fine-grained analysis of the training set is needed, 
perhaps leading to feature re-engineering.

What can be achieved with repeated retraining of models is only one
aspect of improving \emph{interpretability}, a large and crucial
concern in machine learning (see, for example, the general discussions
in~\cite{doshi2017roadmap,Lipton16mythos}, the extensive human
subjects experiments in~\cite{poursabzi2018manipulating}, as well the
many references in these papers). At this level of generality one can
assume that model debugging also falls under interpretability. There
are already some perspectives on interpretability that are better
understood, for example separating model components into ``shape''
functions, one for each feature, in generalized additive models, in
particular for linear and logistic
regression~\cite{LouCG12,CaruanaLGKSE15}. This perspective is
orthogonal to the kind of interpretability we aim to support:
understanding how the learned model parameters depend on the
different groups of samples from the training dataset. 

We did find one approach to interpretability aspects that our work can
be compared against~\cite{koh2017understanding}. It develops an {\em
  influence function} to approximately quantify the influence of a
\emph{single} training sample on the model parameters and prediction
results; this can also be
used for incremental update by estimating the model parameter change
after the removal of one training sample.  \scream{lengthier
  discussion is in Related Work and there is overlap, maybe a bit of
  space can be saved?}  However, our results show (see
Section~\ref{sec: experiment}) that extending the influence function
approach to multiple training samples (for example, all those coming
from a given source) leads to significantly
more inaccurate models than the ones obtained by simply retraining with a subset of the samples. \scream{add that it leads to models that are quite dissimilar or at further distance from the ones obtained by plain retraining}

Searching for an efficient yet accurate approach to incrementally
updating the model after the removal of subsets of training samples, 
we note that the problem can be seen as a {\em data
provenance}~\cite{green2007provenance,buneman2001and,CheneyCT09} question.  
In general, data provenance tracks the dependencies between
input and output data; in particular, the \emph{provenance semiring framework}
\cite{green2007provenance,GreenT17}
has been used for applying incremental updates (specifically deletions)
to views, and more generally, through schema 
mappings~\cite{ives2008orchestra}.

In the semiring framework, output data is annotated with \emph{provenance
polynomials} expressed in terms of provenance tokens that annotate
input data thus making deletion propagation straightforwardly efficient.
%This is done by propagating provenance tokens associated with the
%input tuples through relational algebra operations such as join and
%union to the query result.[[[NO NEED HERE; THIS IS EXPLAINED IN MORE 
%DETAIL IN SECTION 4.1]]]  
The framework has proven quite versatile, allowing for extensions 
to powerful query languages (see references in~\cite{GreenT17}).
Most relevant to the present paper, the framework has been extended to
include the basic linear algebra operations: matrix addition and
multiplication~\cite{yan2016fine} (which was mentioned 
in~\cite{buneman2019data} as a first step in \emph{using data
provenance for interpretability} of machine learning models).
In this extension, as in ~\cite{amsterdamer2011provenance}, the
provenance polynomials play the role of scalars and multiplication
with scalars plays the role of annotating matrices and vectors with
provenance.

In this paper we use the extension of the semiring framework to
basic linear algebra in order to track the provenance of input
samples through the training of logistic regression and linear
regression models using iterative gradient-based methods (GBMs).
In each iteration, we have a gradient-based ``rule'' that updates the 
model parameters. We can annotate the gradient update rule with 
provenance polynomials 
when it is expressed using matrix addition and multiplication. This is
the case when using GBM in linear regression. For logistic regression
we achieve this via piecewise linear interpolation of the non-linear
components in the gradient update rule.

In addition to allowing provenance tracking, the linearization of the
gradient update rule also allows us to separate the contributions of
the training samples from the contributions of the model parameters
(from the previous iteration).  As a result, the effect of deleting
training samples upon the gradient update rule can be obtained by
setting the provenance tokens corresponding to those samples to zero.
To speed up computation, we are able, for both linear and logistic
regression, to cache, between iterations, intermediate results that
capture only the contribution of the training samples, annotated with
provenance. Propagating the deletions of some of the samples then
comes down to subtracting a portion of these intermediate results.  An
additional subtlety for logistic regression is that the piecewise
linear interpolation uses coefficients which are different in
different iterations and hence need to be tracked in the computation.


\scream{Talk about the optimizations for \sgd\ and \minisgd}
We also noted that with stochastic gradient descent (\sgd) and mini-batch stochastic gradient descent (\minisgd), only a small portion of the training samples are used in each iteration, which can achieve significant speed-ups compared to traditional gradient descent method, thus reducing the performance gains brought by the idea of simply caching the intermediate results in the update rule. But we also observed that the rank of the cached intermediate results is small once the mini-batch size is small in \minisgd\ since the intermediate result represents the sum of multiple \textbf{rank-1} terms (each of which is contributed by one training sample from the mini-batch) and thus its rank should be no more than the mini-batch size. So we determined to decompose the intermediate result for \textbf{dense datasets} into the multiplications of two lower-rank matrix by only keeping the most important components of its singular value decomposition \cite{forsythe1967computer}.
\scream{do we need to say this here? Is the SKIN example using SVD?}


\scream{shortened SKIN example, however, this example is about cleaning}


As we shall see, our provenance-based incremental model update along with the optimizations by leveraging singular value decomposition
leads, when compared to a baseline of just retraining the model
from the updated input data, \scream{please examine carefully what I am saying here}
leads to speed-ups of one to two orders of magnitude for 
most training datasets except \scream{the sparse one where we are
only 10\% faster than the baseline}. What is the practical impact of our results?
For an engineer who needs to retrain just once a model after deleting 
some training samples the practical impact is limited for datasets for which
training takes a few minutes. However, for an engineer who explores 
factors of interpretability by retraining many times with different subsets
of a training dataset even one order of magnitude speed-up reduces exploration
from, say, a several-hour run to a run of a couple of minutes
\scream{see experiment in SECTION \ref{sec: experiment}}. This is precisely
how we envision our method's assistance to interpretability.


\scream{put here the text after SKIN example in the old intro}

\scream{our contributions, edited}


